A rewriting-logic-with-SMT-based formal analysis and parameter synthesis framework for parametric time Petri nets

This paper presents a concrete and a symbolic rewriting logic semantics for parametric time Petri nets with inhibitor arcs (PITPNs), a flexible model of timed systems where parameters are allowed in firing bounds. We prove that our semantics is bisimilar to the "standard" semantics of PITPNs. This allows us to use the rewriting logic tool Maude, combined with SMT solving, to provide sound and complete formal analyses for PITPNs. We develop and implement a new general folding approach for symbolic reachability, so that Maude-with-SMT reachability analysis terminates whenever the parametric state-class graph of the PITPN is finite. Our work opens up the possibility of using the many formal analysis capabilities of Maude -- including full LTL model checking, analysis with user-defined analysis strategies, and even statistical model checking -- for such nets. We illustrate this by explaining how almost all formal analysis and parameter synthesis methods supported by the state-of-the-art PITPN tool Romeo can be performed using Maude with SMT. In addition, we also support analysis and parameter synthesis from parametric initial markings, as well as full LTL model checking and analysis with user-defined execution strategies. Experiments show that our methods outperform Romeo in many cases.

==> benchmarks/table-params.tex <==
\begin{tabular}{lrrrr}
\toprule
\textbf{model} & \textbf{parameters} & \textbf{places} & \textbf{transitions} & \textbf{arcs} \\
\midrule
abitpro & 0 & 12 & 16 & 40 \\
producer_consumer & 1 & 5 & 4 & 10 \\
scheduling & 3 & 6 & 9 & 15 \\
train1 & 0 & 12 & 11 & 33 \\
train2 & 0 & 16 & 17 & 65 \\
tutorial & 2 & 6 & 5 & 12 \\
\bottomrule
\end{tabular}


==> benchmarks/table-times-p0.tex <==
\begin{tabular}{llrrrrrrrrrrrrrrrrr}
\toprule
\textbf{model} & \textbf{place\_reached} & \textbf{romeo(ms)} & \textbf{search-sym\_base\_maude(ms)} & \textbf{search-sym\_yices2\_maude(ms)} & \textbf{search-sym\_z3\_maude(ms)} & \textbf{search-sym\_cvc4\_maude(ms)} & \textbf{search-sym2\_base\_maude(ms)} & \textbf{search-sym2\_yices2\_maude(ms)} & \textbf{search-sym2\_z3\_maude(ms)} & \textbf{search-sym2\_cvc4\_maude(ms)} & \textbf{search-folding\_base\_maude(ms)} & \textbf{search-folding\_yices2\_maude(ms)} & \textbf{search-folding\_z3\_maude(ms)} & \textbf{search-folding\_cvc4\_maude(ms)} & \textbf{folding\_base\_maude(ms)} & \textbf{folding\_yices2\_maude(ms)} & \textbf{folding\_z3\_maude(ms)} & \textbf{folding\_cvc4\_maude(ms)} \\
\midrule
abitpro & P1 & \color{OliveGreen} \bfseries 3.0 & 16.0 & 17.0 & 27.0 & 18.0 & 16.0 & 18.0 & 28.0 & 18.0 & 16.0 & 16.0 & 28.0 & 18.0 & 35.0 & 35.0 & 71.0 & 38.0 \\
abitpro & P2 & \color{OliveGreen} \bfseries 3.0 & 16.0 & 17.0 & 28.0 & 17.0 & 17.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 34.0 & 36.0 & 70.0 & 38.0 \\
abitpro & P3 & \color{OliveGreen} \bfseries 4.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 16.0 & 28.0 & 18.0 & 35.0 & 35.0 & 70.0 & 38.0 \\
abitpro & P4 & \color{OliveGreen} \bfseries 4.0 & 16.0 & 19.0 & 28.0 & 18.0 & 16.0 & 16.0 & 28.0 & 17.0 & 16.0 & 17.0 & 28.0 & 18.0 & 34.0 & 35.0 & 70.0 & 38.0 \\
abitpro & P5 & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 28.0 & 17.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 35.0 & 35.0 & 71.0 & 38.0 \\
abitpro & P6 & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 27.0 & 17.0 & 16.0 & 17.0 & 27.0 & 17.0 & 16.0 & 16.0 & 28.0 & 18.0 & 42.0 & 35.0 & 71.0 & 38.0 \\
abitpro & P7 & \color{OliveGreen} \bfseries 4.0 & 16.0 & 16.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 16.0 & 28.0 & 18.0 & 35.0 & 36.0 & 69.0 & 38.0 \\
abitpro & P8 & \color{OliveGreen} \bfseries 5.0 & 16.0 & 16.0 & 28.0 & 17.0 & 16.0 & 16.0 & 28.0 & 17.0 & 16.0 & 17.0 & 28.0 & 18.0 & 34.0 & 35.0 & 69.0 & 38.0 \\
abitpro & P9 & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 28.0 & 18.0 & 16.0 & 17.0 & 27.0 & 17.0 & 16.0 & 17.0 & 32.0 & 18.0 & 35.0 & 36.0 & 71.0 & 40.0 \\
abitpro & P10 & \color{OliveGreen} \bfseries 4.0 & 16.0 & 17.0 & 27.0 & 17.0 & 16.0 & 16.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 17.0 & 35.0 & 35.0 & 69.0 & 39.0 \\
abitpro & P11 & \color{OliveGreen} \bfseries 4.0 & 16.0 & 17.0 & 28.0 & 17.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 16.0 & 28.0 & 18.0 & 34.0 & 35.0 & 71.0 & 39.0 \\
abitpro & P12 & \color{OliveGreen} \bfseries 5.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 29.0 & 18.0 & 16.0 & 17.0 & 29.0 & 18.0 & 35.0 & 35.0 & 70.0 & 38.0 \\
producer_consumer & itemReady & \color{OliveGreen} \bfseries 2.0 & 15.0 & 16.0 & 29.0 & 18.0 & 16.0 & 16.0 & 29.0 & 17.0 & 16.0 & 16.0 & 29.0 & 17.0 & 33.0 & 34.0 & 68.0 & 37.0 \\
producer_consumer & buffer & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 29.0 & 18.0 & 16.0 & 16.0 & 29.0 & 17.0 & 16.0 & 17.0 & 29.0 & 18.0 & 32.0 & 34.0 & 67.0 & 37.0 \\
producer_consumer & itemReceived & \color{BrickRed} \bfseries TO & \color{OliveGreen} \bfseries 16.0 & \color{OliveGreen} \bfseries 16.0 & 29.0 & 17.0 & \color{OliveGreen} \bfseries 16.0 & \color{OliveGreen} \bfseries 16.0 & 29.0 & 17.0 & \color{OliveGreen} \bfseries 16.0 & \color{OliveGreen} \bfseries 16.0 & 28.0 & 18.0 & 33.0 & 35.0 & 68.0 & 38.0 \\
producer_consumer & readyConsumer & \color{OliveGreen} \bfseries 2.0 & 15.0 & 26.0 & 28.0 & 17.0 & 16.0 & 16.0 & 29.0 & 17.0 & 16.0 & 16.0 & 29.0 & 18.0 & 33.0 & 34.0 & 68.0 & 37.0 \\
producer_consumer & readyProducer & \color{OliveGreen} \bfseries 2.0 & 21.0 & 16.0 & 29.0 & 18.0 & 16.0 & 16.0 & 28.0 & 17.0 & 15.0 & 16.0 & 28.0 & 17.0 & 34.0 & 35.0 & 68.0 & 38.0 \\
scheduling & ready1 & \color{OliveGreen} \bfseries 2.0 & 16.0 & 16.0 & 28.0 & 18.0 & 16.0 & 16.0 & 30.0 & 18.0 & 16.0 & 17.0 & 30.0 & 18.0 & 35.0 & 35.0 & 70.0 & 39.0 \\
scheduling & ready2 & \color{OliveGreen} \bfseries 2.0 & 16.0 & 16.0 & 30.0 & 18.0 & 16.0 & 16.0 & 29.0 & 18.0 & 16.0 & 17.0 & 29.0 & 18.0 & 38.0 & 35.0 & 70.0 & 39.0 \\
scheduling & ready3 & \color{OliveGreen} \bfseries 2.0 & 16.0 & 16.0 & 29.0 & 17.0 & 16.0 & 16.0 & 29.0 & 18.0 & 16.0 & 16.0 & 30.0 & 18.0 & 35.0 & 35.0 & 70.0 & 39.0 \\
scheduling & ending1 & \color{OliveGreen} \bfseries 4.0 & 16.0 & 16.0 & 29.0 & 18.0 & 16.0 & 16.0 & 29.0 & 18.0 & 16.0 & 17.0 & 29.0 & 18.0 & 34.0 & 35.0 & 70.0 & 39.0 \\
scheduling & ending2 & \color{OliveGreen} \bfseries 5.0 & 16.0 & 16.0 & 29.0 & 18.0 & 16.0 & 16.0 & 30.0 & 18.0 & 16.0 & 16.0 & 34.0 & 18.0 & 34.0 & 35.0 & 67.0 & 40.0 \\
scheduling & ending3 & \color{OliveGreen} \bfseries 8.0 & 16.0 & 16.0 & 29.0 & 18.0 & 16.0 & 16.0 & 29.0 & 17.0 & 16.0 & 16.0 & 29.0 & 18.0 & 34.0 & 35.0 & 70.0 & 39.0 \\
train1 & in & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 28.0 & 18.0 & 16.0 & 17.0 & 27.0 & 18.0 & 16.0 & 17.0 & 28.0 & 17.0 & 34.0 & 35.0 & 70.0 & 39.0 \\
train1 & far & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 27.0 & 17.0 & 16.0 & 16.0 & 28.0 & 17.0 & 16.0 & 16.0 & 28.0 & 18.0 & 34.0 & 35.0 & 69.0 & 38.0 \\
train1 & coming & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 28.0 & 17.0 & 16.0 & 16.0 & 28.0 & 18.0 & 17.0 & 16.0 & 28.0 & 18.0 & 35.0 & 35.0 & 69.0 & 38.0 \\
train1 & leaving & \color{OliveGreen} \bfseries 4.0 & 16.0 & 16.0 & 27.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 27.0 & 18.0 & 35.0 & 36.0 & 68.0 & 39.0 \\
train1 & open & \color{OliveGreen} \bfseries 3.0 & 16.0 & 17.0 & 36.0 & 17.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 16.0 & 28.0 & 17.0 & 34.0 & 35.0 & 68.0 & 38.0 \\
train1 & lowering & \color{OliveGreen} \bfseries 3.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 17.0 & 34.0 & 35.0 & 68.0 & 38.0 \\
train1 & raising & \color{OliveGreen} \bfseries 4.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 16.0 & 28.0 & 17.0 & 16.0 & 17.0 & 28.0 & 18.0 & 34.0 & 35.0 & 69.0 & 38.0 \\
train1 & closed & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 34.0 & 35.0 & 69.0 & 38.0 \\
train1 & close1 & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 28.0 & 18.0 & 16.0 & 16.0 & 28.0 & 17.0 & 16.0 & 16.0 & 28.0 & 17.0 & 34.0 & 35.0 & 70.0 & 38.0 \\
train1 & on1 & \color{OliveGreen} \bfseries 3.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 16.0 & 28.0 & 17.0 & 16.0 & 16.0 & 27.0 & 18.0 & 47.0 & 44.0 & 69.0 & 38.0 \\
train1 & left1 & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 27.0 & 18.0 & 16.0 & 16.0 & 28.0 & 17.0 & 16.0 & 16.0 & 28.0 & 18.0 & 34.0 & 35.0 & 69.0 & 38.0 \\
train1 & far1 & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 28.0 & 18.0 & 16.0 & 16.0 & 28.0 & 18.0 & 16.0 & 16.0 & 28.0 & 17.0 & 34.0 & 35.0 & 69.0 & 37.0 \\
train2 & in & \color{OliveGreen} \bfseries 4.0 & 17.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 17.0 & 16.0 & 17.0 & 28.0 & 18.0 & 36.0 & 36.0 & 69.0 & 39.0 \\
train2 & far & \color{OliveGreen} \bfseries 4.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 27.0 & 19.0 & 17.0 & 17.0 & 27.0 & 18.0 & 36.0 & 36.0 & 70.0 & 39.0 \\
train2 & coming & \color{OliveGreen} \bfseries 4.0 & 16.0 & 17.0 & 28.0 & 18.0 & 17.0 & 17.0 & 28.0 & 18.0 & 17.0 & 17.0 & 28.0 & 18.0 & 35.0 & 36.0 & 69.0 & 39.0 \\
train2 & leaving & \color{OliveGreen} \bfseries 5.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 17.0 & 17.0 & 28.0 & 18.0 & 35.0 & 36.0 & 76.0 & 39.0 \\
train2 & open & \color{OliveGreen} \bfseries 4.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 36.0 & 36.0 & 70.0 & 39.0 \\
train2 & lowering & \color{OliveGreen} \bfseries 4.0 & 16.0 & 17.0 & 27.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 36.0 & 36.0 & 70.0 & 39.0 \\
train2 & raising & \color{OliveGreen} \bfseries 5.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 36.0 & 37.0 & 70.0 & 43.0 \\
train2 & closed & \color{OliveGreen} \bfseries 5.0 & 17.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 17.0 & 17.0 & 29.0 & 18.0 & 35.0 & 36.0 & 69.0 & 40.0 \\
train2 & close1 & \color{OliveGreen} \bfseries 4.0 & 16.0 & 17.0 & 28.0 & 18.0 & 17.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 35.0 & 36.0 & 70.0 & 39.0 \\
train2 & on1 & \color{OliveGreen} \bfseries 7.0 & 17.0 & 17.0 & 28.0 & 18.0 & 17.0 & 17.0 & 29.0 & 18.0 & 16.0 & 18.0 & 28.0 & 20.0 & 36.0 & 37.0 & 69.0 & 39.0 \\
train2 & left1 & \color{OliveGreen} \bfseries 8.0 & 17.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 29.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 35.0 & 36.0 & 70.0 & 39.0 \\
train2 & far1 & \color{OliveGreen} \bfseries 3.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 35.0 & 36.0 & 70.0 & 39.0 \\
train2 & close2 & \color{OliveGreen} \bfseries 4.0 & 16.0 & 17.0 & 28.0 & 18.0 & 17.0 & 17.0 & 29.0 & 19.0 & 17.0 & 17.0 & 28.0 & 18.0 & 35.0 & 36.0 & 68.0 & 39.0 \\
train2 & on2 & \color{OliveGreen} \bfseries 5.0 & 17.0 & 17.0 & 29.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 27.0 & 18.0 & 36.0 & 37.0 & 69.0 & 39.0 \\
train2 & left2 & \color{OliveGreen} \bfseries 5.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 17.0 & 17.0 & 29.0 & 18.0 & 36.0 & 36.0 & 70.0 & 40.0 \\
train2 & far2 & \color{OliveGreen} \bfseries 4.0 & 16.0 & 17.0 & 28.0 & 18.0 & 17.0 & 17.0 & 29.0 & 18.0 & 17.0 & 17.0 & 28.0 & 18.0 & 36.0 & 37.0 & 69.0 & 40.0 \\
tutorial & start & \color{OliveGreen} \bfseries 2.0 & 16.0 & 16.0 & 29.0 & 18.0 & 16.0 & 16.0 & 30.0 & 17.0 & 16.0 & 16.0 & 30.0 & 18.0 & 33.0 & 35.0 & 68.0 & 39.0 \\
tutorial & childStart & \color{OliveGreen} \bfseries 3.0 & 16.0 & 20.0 & 30.0 & 18.0 & 16.0 & 16.0 & 29.0 & 17.0 & 16.0 & 17.0 & 30.0 & 18.0 & 34.0 & 35.0 & 68.0 & 38.0 \\
tutorial & fatherCont & \color{OliveGreen} \bfseries 3.0 & 15.0 & 16.0 & 29.0 & 18.0 & 16.0 & 16.0 & 29.0 & 17.0 & 16.0 & 16.0 & 29.0 & 18.0 & 34.0 & 35.0 & 68.0 & 38.0 \\
tutorial & childDone & \color{OliveGreen} \bfseries 3.0 & 16.0 & 17.0 & 29.0 & 18.0 & 16.0 & 16.0 & 29.0 & 18.0 & 16.0 & 16.0 & 29.0 & 17.0 & 35.0 & 34.0 & 71.0 & 38.0 \\
tutorial & fatherDone & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 30.0 & 18.0 & 16.0 & 16.0 & 30.0 & 18.0 & 16.0 & 17.0 & 29.0 & 18.0 & 34.0 & 35.0 & 68.0 & 38.0 \\
tutorial & joined & \color{OliveGreen} \bfseries 4.0 & 16.0 & 16.0 & 29.0 & 18.0 & 16.0 & 16.0 & 29.0 & 18.0 & 15.0 & 16.0 & 28.0 & 17.0 & 34.0 & 34.0 & 69.0 & 38.0 \\
\bottomrule
\end{tabular}


==> benchmarks/table-times-p1.tex <==
\begin{tabular}{llrrrrrrrrrrrrrrrrr}
\toprule
\textbf{model} & \textbf{place\_reached} & \textbf{romeo(ms)} & \textbf{search-sym\_base\_maude(ms)} & \textbf{search-sym\_yices2\_maude(ms)} & \textbf{search-sym\_z3\_maude(ms)} & \textbf{search-sym\_cvc4\_maude(ms)} & \textbf{search-sym2\_base\_maude(ms)} & \textbf{search-sym2\_yices2\_maude(ms)} & \textbf{search-sym2\_z3\_maude(ms)} & \textbf{search-sym2\_cvc4\_maude(ms)} & \textbf{search-folding\_base\_maude(ms)} & \textbf{search-folding\_yices2\_maude(ms)} & \textbf{search-folding\_z3\_maude(ms)} & \textbf{search-folding\_cvc4\_maude(ms)} & \textbf{folding\_base\_maude(ms)} & \textbf{folding\_yices2\_maude(ms)} & \textbf{folding\_z3\_maude(ms)} & \textbf{folding\_cvc4\_maude(ms)} \\
\midrule
abitpro & P1 & \color{OliveGreen} \bfseries 3.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 29.0 & 18.0 & 18.0 & 17.0 & 28.0 & 18.0 & 35.0 & 35.0 & 71.0 & 38.0 \\
abitpro & P2 & \color{OliveGreen} \bfseries 3.0 & 16.0 & 17.0 & 48.0 & 19.0 & 17.0 & 17.0 & 69.0 & 21.0 & 17.0 & 18.0 & 66.0 & 22.0 & 52.0 & 55.0 & 239.0 & 71.0 \\
abitpro & P3 & \color{OliveGreen} \bfseries 3.0 & 23.0 & 25.0 & 1102.0 & 116.0 & 23.0 & 25.0 & 766.0 & 86.0 & 25.0 & 29.0 & 731.0 & 89.0 & 66.0 & 70.0 & 902.0 & 142.0 \\
abitpro & P4 & \color{OliveGreen} \bfseries 3.0 & 28.0 & 35.0 & 2267.0 & 230.0 & 27.0 & 31.0 & 1120.0 & 127.0 & 29.0 & 33.0 & 911.0 & 111.0 & 72.0 & 76.0 & 1207.0 & 176.0 \\
abitpro & P5 & \color{OliveGreen} \bfseries 3.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 16.0 & 28.0 & 17.0 & 16.0 & 17.0 & 28.0 & 18.0 & 35.0 & 36.0 & 71.0 & 38.0 \\
abitpro & P6 & \color{OliveGreen} \bfseries 3.0 & 17.0 & 18.0 & 245.0 & 38.0 & 18.0 & 19.0 & 276.0 & 41.0 & 18.0 & 20.0 & 278.0 & 42.0 & 58.0 & 60.0 & 419.0 & 90.0 \\
abitpro & P7 & \color{OliveGreen} \bfseries 3.0 & 19.0 & 21.0 & 542.0 & 65.0 & 20.0 & 22.0 & 468.0 & 60.0 & 22.0 & 23.0 & 452.0 & 61.0 & 62.0 & 66.0 & 729.0 & 120.0 \\
abitpro & P8 & \color{OliveGreen} \bfseries 3.0 & 41.0 & 50.0 & 4246.0 & 411.0 & 33.0 & 40.0 & 1828.0 & 191.0 & 34.0 & 38.0 & 1257.0 & 149.0 & 82.0 & 91.0 & 1570.0 & 223.0 \\
abitpro & P9 & \color{OliveGreen} \bfseries 3.0 & 17.0 & 18.0 & 53.0 & 20.0 & 17.0 & 19.0 & 72.0 & 23.0 & 17.0 & 18.0 & 67.0 & 22.0 & 53.0 & 55.0 & 236.0 & 72.0 \\
abitpro & P10 & \color{OliveGreen} \bfseries 3.0 & 19.0 & 21.0 & 542.0 & 68.0 & 20.0 & 22.0 & 470.0 & 59.0 & 21.0 & 23.0 & 454.0 & 64.0 & 62.0 & 65.0 & 720.0 & 121.0 \\
abitpro & P11 & \color{OliveGreen} \bfseries 3.0 & 29.0 & 34.0 & 2275.0 & 231.0 & 27.0 & 31.0 & 1130.0 & 124.0 & 29.0 & 33.0 & 912.0 & 109.0 & 72.0 & 76.0 & 1211.0 & 176.0 \\
abitpro & P12 & \color{OliveGreen} \bfseries 3.0 & 63.0 & 81.0 & 7865.0 & 762.0 & 44.0 & 55.0 & 2580.0 & 276.0 & 43.0 & 51.0 & 1640.0 & 194.0 & 90.0 & 100.0 & 1856.0 & 261.0 \\
producer_consumer & itemReady & \color{BrickRed} \bfseries TO & \color{OliveGreen} \bfseries 16.0 & 17.0 & 102.0 & 24.0 & \color{OliveGreen} \bfseries 16.0 & 17.0 & 63.0 & 21.0 & \color{OliveGreen} \bfseries 16.0 & 17.0 & 66.0 & 21.0 & 51.0 & 52.0 & 139.0 & 61.0 \\
producer_consumer & buffer & \color{OliveGreen} \bfseries 4.0 & 17.0 & 18.0 & 203.0 & 33.0 & 17.0 & 17.0 & 130.0 & 29.0 & 17.0 & 18.0 & 132.0 & 29.0 & 51.0 & 53.0 & 189.0 & 66.0 \\
producer_consumer & itemReceived & \color{BrickRed} \bfseries TO & 18.0 & 18.0 & 253.0 & 40.0 & \color{OliveGreen} \bfseries 17.0 & 19.0 & 204.0 & 36.0 & 18.0 & 19.0 & 214.0 & 37.0 & 54.0 & 56.0 & 262.0 & 77.0 \\
producer_consumer & readyConsumer & \color{BrickRed} \bfseries TO & \color{OliveGreen} \bfseries 16.0 & \color{OliveGreen} \bfseries 16.0 & 30.0 & 17.0 & \color{OliveGreen} \bfseries 16.0 & \color{OliveGreen} \bfseries 16.0 & 29.0 & 18.0 & \color{OliveGreen} \bfseries 16.0 & \color{OliveGreen} \bfseries 16.0 & 29.0 & 17.0 & 33.0 & 34.0 & 67.0 & 37.0 \\
producer_consumer & readyProducer & \color{BrickRed} \bfseries TO & \color{OliveGreen} \bfseries 15.0 & 16.0 & 29.0 & 17.0 & 16.0 & 16.0 & 29.0 & 17.0 & 16.0 & 16.0 & 29.0 & 17.0 & 33.0 & 34.0 & 68.0 & 37.0 \\
scheduling & ready1 & 27.0 & \color{OliveGreen} \bfseries 16.0 & \color{OliveGreen} \bfseries 16.0 & 29.0 & 18.0 & \color{OliveGreen} \bfseries 16.0 & \color{OliveGreen} \bfseries 16.0 & 29.0 & 17.0 & \color{OliveGreen} \bfseries 16.0 & \color{OliveGreen} \bfseries 16.0 & 29.0 & 18.0 & 34.0 & 35.0 & 70.0 & 45.0 \\
scheduling & ready2 & 26.0 & \color{OliveGreen} \bfseries 16.0 & \color{OliveGreen} \bfseries 16.0 & 30.0 & 18.0 & \color{OliveGreen} \bfseries 16.0 & \color{OliveGreen} \bfseries 16.0 & 29.0 & 17.0 & \color{OliveGreen} \bfseries 16.0 & \color{OliveGreen} \bfseries 16.0 & 29.0 & 18.0 & 34.0 & 35.0 & 71.0 & 40.0 \\
scheduling & ready3 & 26.0 & \color{OliveGreen} \bfseries 16.0 & \color{OliveGreen} \bfseries 16.0 & 29.0 & 18.0 & \color{OliveGreen} \bfseries 16.0 & \color{OliveGreen} \bfseries 16.0 & 29.0 & 18.0 & \color{OliveGreen} \bfseries 16.0 & \color{OliveGreen} \bfseries 16.0 & 30.0 & 18.0 & 34.0 & 35.0 & 70.0 & 39.0 \\
scheduling & ending1 & 26.0 & 18.0 & 18.0 & 180.0 & 34.0 & \color{OliveGreen} \bfseries 17.0 & 18.0 & 103.0 & 27.0 & \color{OliveGreen} \bfseries 17.0 & 18.0 & 104.0 & 28.0 & 54.0 & 55.0 & 184.0 & 70.0 \\
scheduling & ending2 & 26.0 & 23.0 & 25.0 & 575.0 & 83.0 & \color{OliveGreen} \bfseries 22.0 & 25.0 & 325.0 & 62.0 & 24.0 & 27.0 & 328.0 & 64.0 & 61.0 & 66.0 & 400.0 & 108.0 \\
scheduling & ending3 & \color{OliveGreen} \bfseries 29.0 & 36.0 & 45.0 & 1266.0 & 190.0 & \color{OliveGreen} \bfseries 29.0 & 37.0 & 569.0 & 116.0 & 35.0 & 41.0 & 577.0 & 117.0 & 81.0 & 90.0 & 639.0 & 171.0 \\
train1 & in & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 49.0 & 20.0 & 16.0 & 17.0 & 66.0 & 21.0 & 17.0 & 17.0 & 66.0 & 21.0 & 52.0 & 54.0 & 196.0 & 67.0 \\
train1 & far & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 28.0 & 18.0 & 16.0 & 16.0 & 28.0 & 17.0 & 16.0 & 16.0 & 28.0 & 17.0 & 34.0 & 35.0 & 69.0 & 38.0 \\
train1 & coming & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 48.0 & 19.0 & 16.0 & 17.0 & 66.0 & 21.0 & 17.0 & 17.0 & 67.0 & 22.0 & 52.0 & 54.0 & 197.0 & 66.0 \\
train1 & leaving & \color{OliveGreen} \bfseries 3.0 & 34.0 & 40.0 & 2790.0 & 272.0 & 22.0 & 25.0 & 663.0 & 82.0 & 24.0 & 27.0 & 677.0 & 83.0 & 62.0 & 66.0 & 753.0 & 127.0 \\
train1 & open & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 28.0 & 17.0 & 16.0 & 16.0 & 28.0 & 17.0 & 16.0 & 16.0 & 28.0 & 17.0 & 34.0 & 35.0 & 68.0 & 37.0 \\
train1 & lowering & \color{OliveGreen} \bfseries 3.0 & 17.0 & 18.0 & 193.0 & 33.0 & 17.0 & 18.0 & 211.0 & 35.0 & 18.0 & 19.0 & 215.0 & 37.0 & 53.0 & 56.0 & 311.0 & 76.0 \\
train1 & raising & \color{OliveGreen} \bfseries 3.0 & 37.0 & 45.0 & 3288.0 & 308.0 & 24.0 & 27.0 & 831.0 & 99.0 & 27.0 & 30.0 & 847.0 & 100.0 & 68.0 & 72.0 & 885.0 & 153.0 \\
train1 & closed & \color{OliveGreen} \bfseries 3.0 & 20.0 & 22.0 & 759.0 & 82.0 & 18.0 & 20.0 & 350.0 & 49.0 & 19.0 & 21.0 & 357.0 & 50.0 & 56.0 & 59.0 & 423.0 & 90.0 \\
train1 & close1 & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 46.0 & 19.0 & 17.0 & 17.0 & 66.0 & 21.0 & 16.0 & 17.0 & 68.0 & 22.0 & 53.0 & 54.0 & 198.0 & 66.0 \\
train1 & on1 & \color{OliveGreen} \bfseries 3.0 & 25.0 & 29.0 & 1606.0 & 159.0 & 20.0 & 22.0 & 483.0 & 64.0 & 21.0 & 23.0 & 490.0 & 65.0 & 58.0 & 61.0 & 532.0 & 102.0 \\
train1 & left1 & \color{OliveGreen} \bfseries 3.0 & 31.0 & 37.0 & 2436.0 & 231.0 & 21.0 & 24.0 & 603.0 & 74.0 & 23.0 & 25.0 & 619.0 & 77.0 & 61.0 & 64.0 & 644.0 & 115.0 \\
train1 & far1 & \color{OliveGreen} \bfseries 3.0 & 16.0 & 16.0 & 28.0 & 17.0 & 16.0 & 16.0 & 28.0 & 17.0 & 16.0 & 16.0 & 28.0 & 17.0 & 34.0 & 35.0 & 69.0 & 38.0 \\
train2 & in & \color{OliveGreen} \bfseries 4.0 & 17.0 & 18.0 & 49.0 & 20.0 & 17.0 & 18.0 & 65.0 & 21.0 & 18.0 & 18.0 & 67.0 & 22.0 & 57.0 & 58.0 & 263.0 & 74.0 \\
train2 & far & \color{OliveGreen} \bfseries 3.0 & 16.0 & 17.0 & 28.0 & 18.0 & 17.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 27.0 & 18.0 & 36.0 & 36.0 & 69.0 & 39.0 \\
train2 & coming & \color{OliveGreen} \bfseries 5.0 & 17.0 & 17.0 & 48.0 & 20.0 & 17.0 & 18.0 & 67.0 & 22.0 & 18.0 & 18.0 & 68.0 & 22.0 & 55.0 & 57.0 & 262.0 & 74.0 \\
train2 & leaving & \color{OliveGreen} \bfseries 5.0 & 233.0 & 304.0 & 26847.0 & 2553.0 & 67.0 & 83.0 & 3880.0 & 434.0 & 97.0 & 114.0 & 3990.0 & 471.0 & 243.0 & 295.0 & 4999.0 & 803.0 \\
train2 & open & \color{OliveGreen} \bfseries 5.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 17.0 & 17.0 & 28.0 & 18.0 & 35.0 & 37.0 & 70.0 & 39.0 \\
train2 & lowering & \color{OliveGreen} \bfseries 5.0 & 18.0 & 19.0 & 250.0 & 38.0 & 19.0 & 20.0 & 282.0 & 43.0 & 20.0 & 21.0 & 285.0 & 44.0 & 65.0 & 68.0 & 613.0 & 115.0 \\
train2 & raising & \color{OliveGreen} \bfseries 5.0 & 346.0 & 454.0 & 38953.0 & 3784.0 & 113.0 & 147.0 & 6987.0 & 801.0 & 189.0 & 224.0 & 7158.0 & 890.0 & 372.0 & 468.0 & 7564.0 & 1255.0 \\
train2 & closed & \color{OliveGreen} \bfseries 5.0 & 30.0 & 34.0 & 2036.0 & 201.0 & 23.0 & 26.0 & 678.0 & 83.0 & 25.0 & 28.0 & 690.0 & 84.0 & 77.0 & 85.0 & 1136.0 & 184.0 \\
train2 & close1 & \color{OliveGreen} \bfseries 5.0 & 16.0 & 17.0 & 50.0 & 20.0 & 17.0 & 18.0 & 66.0 & 22.0 & 17.0 & 18.0 & 66.0 & 22.0 & 55.0 & 57.0 & 268.0 & 74.0 \\
train2 & on1 & \color{OliveGreen} \bfseries 5.0 & 69.0 & 87.0 & 7763.0 & 710.0 & 31.0 & 36.0 & 1406.0 & 161.0 & 37.0 & 43.0 & 1419.0 & 162.0 & 100.0 & 113.0 & 1864.0 & 283.0 \\
train2 & left1 & \color{OliveGreen} \bfseries 5.0 & 160.0 & 208.0 & 18863.0 & 1789.0 & 45.0 & 54.0 & 2447.0 & 267.0 & 59.0 & 68.0 & 2492.0 & 281.0 & 148.0 & 175.0 & 3057.0 & 470.0 \\
train2 & far1 & \color{OliveGreen} \bfseries 5.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 17.0 & 17.0 & 28.0 & 18.0 & 35.0 & 37.0 & 70.0 & 39.0 \\
train2 & close2 & \color{OliveGreen} \bfseries 5.0 & 17.0 & 18.0 & 164.0 & 31.0 & 18.0 & 18.0 & 177.0 & 31.0 & 19.0 & 19.0 & 183.0 & 32.0 & 56.0 & 57.0 & 258.0 & 74.0 \\
train2 & on2 & \color{OliveGreen} \bfseries 5.0 & 80.0 & 103.0 & 9244.0 & 848.0 & 39.0 & 47.0 & 2169.0 & 240.0 & 46.0 & 53.0 & 2206.0 & 241.0 & 98.0 & 112.0 & 1861.0 & 279.0 \\
train2 & left2 & \color{OliveGreen} \bfseries 5.0 & 181.0 & 237.0 & 21201.0 & 2004.0 & 56.0 & 69.0 & 3554.0 & 378.0 & 70.0 & 85.0 & 3618.0 & 395.0 & 148.0 & 173.0 & 2991.0 & 461.0 \\
train2 & far2 & \color{OliveGreen} \bfseries 5.0 & 16.0 & 17.0 & 29.0 & 18.0 & 17.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 36.0 & 36.0 & 69.0 & 39.0 \\
tutorial & start & \color{OliveGreen} \bfseries 4.0 & 16.0 & 16.0 & 29.0 & 18.0 & 16.0 & 16.0 & 29.0 & 18.0 & 16.0 & 16.0 & 30.0 & 18.0 & 34.0 & 35.0 & 68.0 & 39.0 \\
tutorial & childStart & \color{BrickRed} \bfseries TO & \color{OliveGreen} \bfseries 16.0 & \color{OliveGreen} \bfseries 16.0 & 49.0 & 20.0 & 17.0 & 17.0 & 66.0 & 21.0 & 17.0 & 17.0 & 66.0 & 22.0 & 53.0 & 60.0 & 148.0 & 62.0 \\
tutorial & fatherCont & \color{BrickRed} \bfseries TO & \color{OliveGreen} \bfseries 16.0 & 17.0 & 49.0 & 19.0 & \color{OliveGreen} \bfseries 16.0 & 17.0 & 65.0 & 22.0 & 17.0 & 17.0 & 67.0 & 22.0 & 52.0 & 53.0 & 147.0 & 62.0 \\
tutorial & childDone & \color{BrickRed} \bfseries TO & 18.0 & 18.0 & 234.0 & 38.0 & \color{OliveGreen} \bfseries 17.0 & 18.0 & 139.0 & 30.0 & \color{OliveGreen} \bfseries 17.0 & 19.0 & 157.0 & 30.0 & 53.0 & 56.0 & 235.0 & 73.0 \\
tutorial & fatherDone & \color{BrickRed} \bfseries TO & \color{OliveGreen} \bfseries 18.0 & \color{OliveGreen} \bfseries 18.0 & 252.0 & 39.0 & \color{OliveGreen} \bfseries 18.0 & 19.0 & 159.0 & 32.0 & \color{OliveGreen} \bfseries 18.0 & \color{OliveGreen} \bfseries 18.0 & 163.0 & 32.0 & 54.0 & 57.0 & 227.0 & 75.0 \\
tutorial & joined & \color{BrickRed} \bfseries TO & \color{OliveGreen} \bfseries 19.0 & 22.0 & 567.0 & 69.0 & 20.0 & 21.0 & 388.0 & 58.0 & 21.0 & 23.0 & 391.0 & 59.0 & 58.0 & 61.0 & 409.0 & 96.0 \\
\bottomrule
\end{tabular}


==> benchmarks/table-times-p2.tex <==
\begin{tabular}{llrrrrrrrrrrrrrrrrr}
\toprule
\textbf{model} & \textbf{place\_reached} & \textbf{romeo(ms)} & \textbf{search-sym\_base\_maude(ms)} & \textbf{search-sym\_yices2\_maude(ms)} & \textbf{search-sym\_z3\_maude(ms)} & \textbf{search-sym\_cvc4\_maude(ms)} & \textbf{search-sym2\_base\_maude(ms)} & \textbf{search-sym2\_yices2\_maude(ms)} & \textbf{search-sym2\_z3\_maude(ms)} & \textbf{search-sym2\_cvc4\_maude(ms)} & \textbf{search-folding\_base\_maude(ms)} & \textbf{search-folding\_yices2\_maude(ms)} & \textbf{search-folding\_z3\_maude(ms)} & \textbf{search-folding\_cvc4\_maude(ms)} & \textbf{folding\_base\_maude(ms)} & \textbf{folding\_yices2\_maude(ms)} & \textbf{folding\_z3\_maude(ms)} & \textbf{folding\_cvc4\_maude(ms)} \\
\midrule
abitpro & P1 & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 62.0 & 77.0 & 2381.0 & 295.0 & 99.0 & 115.0 & 2367.0 & 320.0 \\
abitpro & P2 & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 61.0 & 76.0 & 2376.0 & 294.0 & 99.0 & 114.0 & 2377.0 & 346.0 \\
abitpro & P3 & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 61.0 & 76.0 & 2383.0 & 293.0 & 100.0 & 114.0 & 2631.0 & 345.0 \\
abitpro & P4 & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 61.0 & 75.0 & 2405.0 & 292.0 & 99.0 & 115.0 & 2379.0 & 346.0 \\
abitpro & P5 & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 62.0 & 76.0 & 2379.0 & 294.0 & 100.0 & 115.0 & 2382.0 & 324.0 \\
abitpro & P6 & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 61.0 & 77.0 & 2383.0 & 291.0 & 99.0 & 114.0 & 2369.0 & 322.0 \\
abitpro & P7 & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 62.0 & 76.0 & 2399.0 & 290.0 & 99.0 & 114.0 & 2380.0 & 321.0 \\
abitpro & P8 & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 61.0 & 75.0 & 2399.0 & 291.0 & 99.0 & 115.0 & 2381.0 & 344.0 \\
abitpro & P9 & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 61.0 & 76.0 & 2399.0 & 293.0 & 99.0 & 113.0 & 2363.0 & 323.0 \\
abitpro & P10 & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 64.0 & 77.0 & 2385.0 & 297.0 & 100.0 & 116.0 & 2382.0 & 333.0 \\
abitpro & P11 & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 62.0 & 76.0 & 2396.0 & 297.0 & 100.0 & 115.0 & 2403.0 & 322.0 \\
abitpro & P12 & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 64.0 & 78.0 & 2381.0 & 294.0 & 100.0 & 114.0 & 2395.0 & 324.0 \\
producer_consumer & itemReady & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO \\
producer_consumer & buffer & \color{BrickRed} \bfseries TO & 22.0 & 26.0 & 794.0 & 98.0 & \color{OliveGreen} \bfseries 19.0 & 20.0 & 284.0 & 47.0 & \color{OliveGreen} \bfseries 19.0 & 21.0 & 282.0 & 46.0 & 59.0 & 64.0 & 415.0 & 103.0 \\
producer_consumer & itemReceived & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO \\
producer_consumer & readyConsumer & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO \\
producer_consumer & readyProducer & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO \\
scheduling & ready1 & \color{OliveGreen} \bfseries 27.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 32656.0 & 43143.0 & 129108.0 & 81343.0 & 3400.0 & 4603.0 & 14503.0 & 8609.0 \\
scheduling & ready2 & \color{OliveGreen} \bfseries 26.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 32187.0 & 43207.0 & 127100.0 & 81435.0 & 3408.0 & 4615.0 & 14118.0 & 8560.0 \\
scheduling & ready3 & \color{OliveGreen} \bfseries 26.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 32369.0 & 43274.0 & 129730.0 & 81265.0 & 3414.0 & 4597.0 & 14453.0 & 8664.0 \\
scheduling & ending1 & \color{OliveGreen} \bfseries 26.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 32128.0 & 43040.0 & 130155.0 & 81234.0 & 3418.0 & 4580.0 & 14466.0 & 8580.0 \\
scheduling & ending2 & \color{OliveGreen} \bfseries 26.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 32118.0 & 43494.0 & 127874.0 & 80943.0 & 3427.0 & 4606.0 & 14539.0 & 8573.0 \\
scheduling & ending3 & \color{OliveGreen} \bfseries 26.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 32289.0 & 43805.0 & 129074.0 & 81029.0 & 3409.0 & 4618.0 & 14528.0 & 8696.0 \\
train1 & in & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 45.0 & 54.0 & 1447.0 & 186.0 & 83.0 & 93.0 & 1389.0 & 232.0 \\
train1 & far & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 45.0 & 53.0 & 1452.0 & 186.0 & 80.0 & 91.0 & 1402.0 & 220.0 \\
train1 & coming & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 45.0 & 54.0 & 1456.0 & 188.0 & 80.0 & 91.0 & 1372.0 & 219.0 \\
train1 & leaving & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 45.0 & 53.0 & 1448.0 & 191.0 & 81.0 & 90.0 & 1372.0 & 221.0 \\
train1 & open & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 45.0 & 53.0 & 1447.0 & 186.0 & 81.0 & 91.0 & 1384.0 & 219.0 \\
train1 & lowering & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 45.0 & 54.0 & 1448.0 & 186.0 & 82.0 & 90.0 & 1372.0 & 223.0 \\
train1 & raising & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 45.0 & 54.0 & 1458.0 & 186.0 & 81.0 & 92.0 & 1366.0 & 233.0 \\
train1 & closed & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 45.0 & 54.0 & 1466.0 & 186.0 & 81.0 & 92.0 & 1377.0 & 222.0 \\
train1 & close1 & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 46.0 & 55.0 & 1461.0 & 188.0 & 81.0 & 92.0 & 1369.0 & 233.0 \\
train1 & on1 & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 45.0 & 53.0 & 1449.0 & 187.0 & 80.0 & 91.0 & 1382.0 & 219.0 \\
train1 & left1 & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 46.0 & 53.0 & 1452.0 & 188.0 & 81.0 & 91.0 & 1372.0 & 220.0 \\
train1 & far1 & \color{OliveGreen} \bfseries 3.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 45.0 & 54.0 & 1447.0 & 187.0 & 80.0 & 91.0 & 1372.0 & 220.0 \\
train2 & in & \color{OliveGreen} \bfseries 5.0 & 19.0 & 20.0 & 341.0 & 46.0 & 20.0 & 21.0 & 373.0 & 51.0 & 21.0 & 22.0 & 378.0 & 51.0 & 63.0 & 68.0 & 623.0 & 116.0 \\
train2 & far & \color{OliveGreen} \bfseries 5.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 28.0 & 18.0 & 16.0 & 17.0 & 27.0 & 18.0 & 35.0 & 36.0 & 71.0 & 39.0 \\
train2 & coming & \color{OliveGreen} \bfseries 5.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 800.0 & 1043.0 & 15307.0 & 2735.0 \\
train2 & leaving & \color{OliveGreen} \bfseries 5.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 801.0 & 1039.0 & 15300.0 & 2828.0 \\
train2 & open & \color{OliveGreen} \bfseries 5.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 803.0 & 1033.0 & 15236.0 & 2745.0 \\
train2 & lowering & \color{OliveGreen} \bfseries 5.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 799.0 & 1040.0 & 15239.0 & 2704.0 \\
train2 & raising & \color{OliveGreen} \bfseries 5.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 800.0 & 1035.0 & 15349.0 & 2821.0 \\
train2 & closed & \color{OliveGreen} \bfseries 5.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 802.0 & 1036.0 & 15185.0 & 2825.0 \\
train2 & close1 & \color{OliveGreen} \bfseries 5.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 799.0 & 1042.0 & 15751.0 & 2818.0 \\
train2 & on1 & \color{OliveGreen} \bfseries 5.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 801.0 & 1029.0 & 15341.0 & 2728.0 \\
train2 & left1 & \color{OliveGreen} \bfseries 5.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 808.0 & 1040.0 & 15203.0 & 2732.0 \\
train2 & far1 & \color{OliveGreen} \bfseries 5.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 796.0 & 1043.0 & 15257.0 & 2735.0 \\
train2 & close2 & \color{OliveGreen} \bfseries 5.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 800.0 & 1033.0 & 15253.0 & 2836.0 \\
train2 & on2 & \color{OliveGreen} \bfseries 5.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 797.0 & 1034.0 & 15229.0 & 2739.0 \\
train2 & left2 & \color{OliveGreen} \bfseries 5.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 803.0 & 1035.0 & 15283.0 & 2743.0 \\
train2 & far2 & \color{OliveGreen} \bfseries 5.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & 806.0 & 1036.0 & 15282.0 & 2855.0 \\
tutorial & start & \color{BrickRed} \bfseries TO & 22.0 & 25.0 & 846.0 & 100.0 & \color{OliveGreen} \bfseries 21.0 & 24.0 & 519.0 & 73.0 & 24.0 & 26.0 & 545.0 & 75.0 & 60.0 & 63.0 & 464.0 & 105.0 \\
tutorial & childStart & \color{BrickRed} \bfseries TO & 31.0 & 38.0 & 1899.0 & 209.0 & \color{OliveGreen} \bfseries 25.0 & 29.0 & 750.0 & 104.0 & 28.0 & 33.0 & 784.0 & 108.0 & 67.0 & 72.0 & 653.0 & 136.0 \\
tutorial & fatherCont & \color{BrickRed} \bfseries TO & 31.0 & 38.0 & 1903.0 & 213.0 & \color{OliveGreen} \bfseries 25.0 & 29.0 & 756.0 & 106.0 & 28.0 & 33.0 & 794.0 & 109.0 & 68.0 & 72.0 & 649.0 & 137.0 \\
tutorial & childDone & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{OliveGreen} \bfseries 19647.0 & 28398.0 & \color{BrickRed} \bfseries TO & 96507.0 & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO \\
tutorial & fatherDone & \color{BrickRed} \bfseries TO & 11461.0 & 16013.0 & \color{BrickRed} \bfseries TO & 84698.0 & \color{OliveGreen} \bfseries 531.0 & 792.0 & 15192.0 & 3261.0 & 1182.0 & 1457.0 & 16299.0 & 3948.0 & 756.0 & 982.0 & 5480.0 & 1985.0 \\
tutorial & joined & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO & \color{BrickRed} \bfseries TO \\
\bottomrule
\end{tabular}


==> benchmarks/table-times-safety.tex <==
\begin{tabular}{lrrrrr}
\toprule
\textbf{model} & \textbf{romeo(ms)} & \textbf{AG-synthesis\_base\_maude(ms)} & \textbf{AG-synthesis\_yices2\_maude(ms)} & \textbf{AG-synthesis\_z3\_maude(ms)} & \textbf{AG-synthesis\_cvc4\_maude(ms)} \\
\midrule
abitpro & \color{OliveGreen} \bfseries 3.0 & 107.0 & 125.0 & 2324.0 & 357.0 \\
producer_consumer & \color{OliveGreen} \bfseries 5.0 & 79.0 & 86.0 & 835.0 & 174.0 \\
scheduling & \color{OliveGreen} \bfseries 84.0 & 3694.0 & 5041.0 & 14939.0 & 9684.0 \\
train1 & \color{OliveGreen} \bfseries 3.0 & 94.0 & 100.0 & 1358.0 & 237.0 \\
train2 & \color{OliveGreen} \bfseries 4.0 & 41.0 & 46.0 & 87.0 & 46.0 \\
tutorial & \color{OliveGreen} \bfseries 4.0 & 65.0 & 70.0 & 496.0 & 114.0 \\
\bottomrule
\end{tabular}

